Exploiting Network Loss for Distributed Approximate Computing with NetApprox

Many data center applications such as machine learning and big data analytics can complete their analysis without processing the complete set of data. While extensive approximate-aware optimizations have been proposed at hardware, programming language, and application levels. However, to date, the approximate computing optimizations have ignored the network layer. We propose NetApprox, which to the best of our knowledge, is the first approximate-aware network layer comprising transport-layer protocol, network resource allocation schemes, and scheduling/priority-assignment policies. Building on the observation that approximate applications can tolerate loss, NetApprox's main insights are to aggressively send approximate traffic (which improves the performance of approximate applications) and to minimize the network resources allocated to approximate traffic (which simultaneously limits the impact of aggressive approximate traffic while freeing up resources that, in turn, improve non-approximate applications' performance). We ported Flink, Kafka, Spark, and PyTorch to NetApprox and evaluated NetApprox with both large-scale simulation and real implementation. Our evaluation results show that NetApprox improves job completion times by up to 80% compared to network-oblivious approximation solutions, and improves the performance of co-running non-approximate workloads by 79%.

==> designchoices.tex <==
\section{Approximate-Aware Network Design}
\label{sec:approx-aware-design}

This section presents a case for incorporating approximate computing and its inherent slack tolerance into the network design, which, in turn, motivates \sysname.
Our key argument is that approximate-computing awareness %, {\em \sysname}, 
can provide the network with additional degrees of freedom in resource allocation 
and scheduling decisions, which will translate into performance improvements along both approximate and regular (non-approximate) applications.


\textit{How should one build a network system for approximate computing?}
Intuitively, we can integrate approximate computing into the network layer's design to exploit approximate computation's inherent slack in one of two ways:
1) by allowing (or letting) data drop to happen within the network,
and 2) by allocating fewer network resources to approximate traffic than non-approximate traffic.
Before presenting \sysname, we first explore several design options for these two dimensions
and discuss why simple designs are insufficient.

%\subsection{Approximate-Aware Transport Design Space}
%\label{sec:transport-design}
%Note: we assume that any form of network-supported approximate computing will build on EarlySend and SenderSideSampling. 
%Given the plethora of existing techniques to address both configuration changes and in-network sampling, 

\subsection{Network support for Approximate Computing}
\label{sec:transport-design-space}
There are two ways to integrate approximate computing into the networking layer: either at the transport or within the network.

\textbf{Transport layer:} We can augment either TCP or UDP protocols to dynamically adjust sending rate to ensure that the current packet loss approximates the specified target loss rate. In this scenario, the protocols will increase the sending rate if the current loss is lower than the target and vice-versa.  On the one hand, there are several challenges: TCP (and reliable protocols) will aggressively retransmit packets that contradict the goal of tolerating more losses.  On the other hand, we can change UDP to only retransmits packets at the end of the connection if sufficient packets have not been delivered to achieve the application specified target.  

\yiying{It's still unclear why the second way (UDP + retransmission at the end) is insufficient.}
\theo{This would unnecessarily send too much traffic (waste resources) and can cause starvation.}

We note that these modifications are inefficient: First, the available capacity of the network constantly changes, and this can lead to burst losses which will impact the applications slack (or instantaneous target loss rate). We need an information rate-adaptation algorithm that is both aware of the network's state (i.e., congestion) and the application's instantaneous target loss rate. \yiying{We need to find a place to better describe the difference between instantaneous target loss rate and the final target loss rate.}
Second, when the application is retransmitting packets, we have the opportunity to retransmit in an order that improves performance. However, existing protocols will default to inorder delivery.

\yiying{Add the discussion that we can be more aggressive on estimating network capacity, because we can tolerate loss}

\if 0
\textbf{Network Layer:} We can have the application mark a subset of packets -- precisely, a subset mark a subset of packets that is equivalent to the target loss rate. Given these markings, the network can use these markings to determine which packet to drop when the network is congested. A key challenge with this approach is that approximate traffic will use up excessive amounts of network buffers. This implies a need to provides in-network isolation and protection mechanisms.
\yiying{I don't really get what this paragraph is about...}
\fi

% We first explore the design space of the transport layer, starting with examining whether or not existing transports can work well for approximate applications.

% \boldparagraph{Problems with Reliable Transport.} 
% Existing approximate computing systems all sit on a reliable transport layer which is, however, a mismatch for approximate computing. 
% %\sy{(I feel the transition is somehow weird here - we mention allowing data drop to happen within the network as the first point at the end of the last paragraph, but we start from discussing reliable transport here.)}
% \theonote{cut expansion}
% % as it ensures the delivery of every packet (through retransmission),
% % incurring unnecessary performance overhead, especially when the receiver may selectively delete or sample data instead of processing them.

% To illustrate the problem with existing reliable transports, \eg, TCP, consider an approximate-aware extension to TCP, which uses information about the application's slack and network congestion to determine the sending rate. 
% Let us further assume that this transport could somehow set the ``perfect'' sending rate, which as we will show in \S\ref{sec:atp}, is challenging.
% There is still a critical problem: TCP's recovery mechanism is unaware of the application's ability to tolerate some loss (i.e., application's slack) and will attempt to recover from every lost packet, which is unnecessary and will slow down transfer completion time.  
% %For any reliable transport to be approximate-aware, the protocol must adjust the sending rate \emph{and} loss recovery mechanisms to incorporate knowledge about slack.

% \boldparagraph{Problems with Unreliable Transport.}
% A seemingly possible design is to use raw UDP and let the network drop packets based on its congestion state.
% Doing so, unfortunately, can impact both the accuracy and the performance of the approximate application.
% When the network is heavily congested, UDP will drop too many packets and will not meet the application's desired accuracy.\theo{should we add a forward pointer to section 6 here?}
% On the other end of the spectrum, when the network is not congested, UDP will send all traffic at a predefined rate, \yiying{Theo: why would there be a predefined rate with UDP?} missing the opportunity to aggressively sending more data to fully utilize the network.

% Similar to our TCP analysis, consider an approximate-aware extension to UDP that could somehow set an ideal sending rate according to application's slack tolerance and network congestion.
% The critical issue is that without data retransmission (\ie, no buffering of un-acknowledged data), unreliable transports have to wait for new data to be ready (passed by applications), which could delay the completion of a job.
% Worse, when not enough new data is available, application-required accuracy could be violated.
% %An improved design builds on UDP and uses information about application's slack and network state to determine sending rate. While this approach dynamically adapts and fully utilizes the network, 
% %without retransmitting data, this approach suffers from a similar problem as the overly aggressive UDP-based approach discussed earlier.  
% %to uniformly drop packets at a fixed rate before sending them with UDP (similar to \midsend) and to start sending the data as soon as the data is ready at the sender (similar to EarlySend). 
% %\yiying{Theo, I don't get this. Is this one approach that combines \midsend\ and EarlySend (and how?) or two approahces, one like \midsend, one like EarlySend?}\theo{I changed this paragraph. instead of trying to tie this to EarlySend/MidSend, i'm just making the UDP naive network/slack aware}
% % This approach suffers from a similar problem \yiying{similar to what?} because it doesn't explicitly tie the network's drop rate to the application's inherent slack. 
% % We must either drop additional packets at the receiver when the drop rate is too low or retransmit lost packets when the drop rate is too high.
% % and consequently dropping more packets at the receiver if drop due to congestion is not enough 
% % and by retransmitting packets if congestion caused too much drop.

\boldparagraph{Insights.} 
There are two fundamental features that an approximate-aware transport layer should have which are not supported in any of today's transports.
First, it should set sending rates that can judiciously match network loss to applications' slack tolerance, \ie, send slightly higher than network capacity to create just the right amount of potential packet loss that could still meet user-specified application accuracy.
Second, it should be able to choose between retransmitting lost packets (\ie, TCP-like) and transmitting (future) new packets (\ie, UDP-like), whichever yields better application job completion time, since most approximate applications do not care about either the ordering of received data or which data is lost as long as enough data is received\footnote{With some caveats, see \S\ref{sec:group-sampling}}.
%From the above analysis, we see that neither TCP or UDP fit approximate computing.
%Thus, approximate computing demands a new transport layer, one that is \emph{partially reliable} 
%and can judiciously incorporate network loss to better utilize approximate applications' slack tolerance. %the slack inherent within approximate applications better.
%The sending rates that such a transport sets should be aggressive but still controlled, \ie, slightly higher than network capacity to create just the right amount of potential packet loss that could still meet user-specified application accuracy.

%\input{fig-network-design}

\subsection{Network Resource Allocation Designs}
\label{sec:switch-design-space}
%\subsection{Strawman Approach.}

Today's network does not treat approximate traffic differently when assigning network resources.
However, approximate computing opens new opportunities and challenges in designing network resource allocation such as switch priority queue assignment and buffer space allocation.
First, there is an opportunity to shift network resources from approximate workloads to non-approximate workloads 
(\eg, assigning lower switch priority queue and/or less switch buffer space to approximate traffic).
Doing so could potentially improve the performance of non-approximate applications at the cost of causing more packet loss for approximate workloads.
This cost is acceptable, in fact embraced, by approximate applications because of their inherent slack tolerance.
At the same time, there are is a new challenge:
with more aggressive sending rates, approximate traffic could (unfairly) occupy large network resources, affecting other traffic.
Moreover, unlike non-approximate workloads, different approximate workloads have different slack tolerance (and thus different amount of resources they potentially need from the network): those that have little slack tolerance (\eg, accept only 5\% data loss) are very different from those that can tolerate huge slack (\eg, can accept 80\% data loss).

\if 0
%The most informed design is a network transport protocol that incorporates both the network state (i.e., congestion) and information about the application's slack characteristics to control the sending rate and determine loss recovery. 
When sending approximate traffic at aggressive rates, a potential challenge would rise: approximate traffic will unfairly use up buffers and link capacity (over non-approximate traffic). 
To solve this issue, we must determine an appropriate queuing mechanism to simultaneously protect non-approximate traffic from approximate and ensure that the network prevents starvation of approximate flows. 
%Figure~\ref{f:inNetworkDesign} shows three possible designs of configuring switch queues and link bandwidth allocation.
%Figure~\ref{f:inNetworkDesign}(A), the status quo, 

Today's network does not differentiate between approximate and non-approximate traffic, which leads to the problem of non-approximate traffic being (unfairly) impacted because of approximate traffic's potential aggressive sending rates.
%
%\boldparagraph{Strawman approaches.}
An improved approach is to separate approximate and non-approximate traffic into different queues. %and assign different weights to them (Figure~\ref{f:inNetworkDesign}(B)). 
%\theo{modified the below, what do you think?}
This design isolates non-approximate traffic from approximate traffic, but it can result in higher latency for non-approximate traffic due to queue build-up. \fi

\boldparagraph{Insights.}
%Today's network systems are agnostic about approximate workloads, treating them in the same way as other workloads.
%However, 
Fundamentally, approximate traffic puts different demands from the network: it requires less network resources (because of its loss tolerance), but if not controlled it could end up unfairly consume too many network resources (because of its aggressive sending rates).
These features demand new switch priority queue and queue buffer space allocation mechanisms. 
%From the analysis above, we see the need for a careful design of switch priority queues and the allocation of buffer space to these queues. 
We want to guarantee that an approximate application's more aggressive sending rates will not affect either non-approximate applications or other approximate applications with a lower slack tolerance (and thus lower sending rate).
This hints at the isolation of traffic and allocation of buffer space to traffic based on their slack tolerance.
Moreover, it is beneficial to allocate more buffer space and assign higher priority to applications that can tolerate less or zero slack.
Recall, approximate traffic that tolerates more slack could use less network resource (buffer space and priority), because packet loss is acceptable for them.

\yiying{may want to mention here or somewhere that unlike TCP which is fully reliable and UDP which is fully unreliable, approximate traffic is not just one category, as different approx degree (loss rate) should be treated differently}
%approximate flows with more network loss than specified by slack must be allocated more resources and vice-versa. Naturally, this addresses starvation because starved traffic with a significant loss can be tolerated by the application's inherent slack and allocated more resources.  
%Whereas fairness for approximate flows is not as different: flows with different slack can tolerate more or less loss. Thus, fairness is defined relative to the application slack -- namely, the network must provide similar resources to flows with similar slack to ensure that they compete fairly with each other. 
%Building on this, flows with more slack should get fewer resources, and similar flows will more slack should get fewer resources.


% Additionally, there are two problems with the above approaches.
% First, many approximate applications have complex accuracy requirements that a simple fixed sample rate cannot express, i.e., applications may not be amendable to uniform drop rates.
% Second, there are several missing performance optimization opportunities in this design. Specifically, we may be able to further leverage the inherent slack of approximate traffic by either allocating fewer queues to them or deprioritizing them; however, either of these approaches requires network cooperation.
%\yiying{Theo, what are these missing opportunities?} \theo{addressed}
%\yiying{Shall we mention any alternative design that is network-aware and on top of TCP? e.g., adjusting sending rate based on congestion and target loss rate?}
%\theo{added this TCP design above before the naive design}

\subsection{Design Goals}
\label{sec:design-goals}
Ultimately, we want approximate applications to complete fast while guaranteeing user-desired accuracies.
At the same time, non-approximate applications should not be affected, or better, could also improve their performance.
To achieve these end goals, an approximate-aware network design should fulfill the following goals:
1) a partially reliable transport that accepts loss, but in a controlled manner,
2) sending rates that adjust to network states and applications' slack tolerance,
3) isolation across approximate and non-approximate traffic and across approximate workloads with different levels of slack tolerance,
4) more network resources allocated to non-approximate workloads and approximate workloads with less slack tolerance \sy{(sentence structure is little awkward.)},
and 5) a working solution that considers production network environments and workloads.
These are the design goals that guide \sysname.

\if 0
%\boldparagraph{Insights.}
%Ideally, we want a situation similar to Figure~\ref{f:inNetworkDesign} (C) 
%where queuing and link capacity is devoted to non-approximate traffic and 
%residual or no resources are used by the approximate traffic. %For example, with knowledge about sampling information and rates, the network can either XXXX.
% the existing design choices and discussing their drawbacks:
The above analysis indicates that a good network design for approximate computing should:
1) dynamically drop packets based on the application's runtime properties and accuracy requirements,
\yiying{Theo: what is runtime properties? should it be network states and application's accuracy req?}
2) adopt a sending rate and retransmission policy that are approximate-application aware and adaptive,
\yiying{Theo: how is 2 different from 1?}
3) isolate network resources for non-approximate and approximate traffic and for approximate traffic with different levels of slack tolerance, 
%ensure starvation-free property for the approximate-traffic,
and 4) allocate more switch buffer space and higher priority to non-approximate traffic and to approximate traffic with little slack tolerance.
%queue allocations to ensure efficient resource allocations and minimize the impact of approximate traffic on non-approximate traffic
%and,
%Moreover, 
\yiying{Something about the dynamic part here? or Sec4?}
These are the design principles that guide \sysname.
%'s transport layer (\atp (Section~\ref{sec:design})). 
\fi



% # \subsection{Approximation-Aware Network Resource Allocation}
% # \label{sec:switch-design}
% # %\boldparagraph{Design space of network allocation.}
% # Approximate applications can tolerate loss while still providing accurate results with reduced network resources.
% # On the other hand, non-approximate applications benefit from having a more significant share of the network's resources. Given these points, our design attempts to answer the following question:
% # \textit{How shall we allocate network resources such as switch buffer spaces and priority queues to approximate and non-approximate applications?}
% # %Our next design question is: what is a principled method to determine good network configurations that allow a system to allocate fewer resources to
% # %approximate traffic and leave more to non-approximate traffic,
% #
% # \boldparagraph{Naive Design.}
% # Figure~\ref{f:inNetworkDesign} shows three possible designs of configuring switch queues and link bandwidth allocation.
% # Figure~\ref{f:inNetworkDesign}(A) mixes approximate and non-approximate traffic in switch queues
% # and only employs fair sharing across them. Doing so gives no favor to non-approximate traffic in network resources.
% # Figure~\ref{f:inNetworkDesign}(B) separates queues for approximate and non-approximate traffic
% # and assigns different weights to them.
% # It improves the configuration of Figure~\ref{f:inNetworkDesign}(A) on bandwidth but still leaves queuing-related issues unaddressed.
% # Figure~\ref{f:inNetworkDesign}(C) eliminates switch queuing for approximate traffic,
% # devoting most switch buffer space and most link capacity to non-approximate traffic.
% # This design is our straw-man design.
% #
% #
% # %\boldparagraph{Insights.}


==> fig-NET-QueueSize.tex <==
{
\begin{figure*}[th]
\begin{minipage}{0.25\textwidth}
\begin{center}
\centerline{\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_Net_Queue_KV_40G.pdf}}
\vspace{-0.01in}
\mycaption{fig-jct-fbkv}{JCT of FBKV.}
{
}
\end{center}
\end{minipage}
\begin{minipage}{0.25\textwidth}
\begin{center}
\centerline{\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_Net_Queue_KV_100G.pdf}}
\vspace{-0.1in}
\mycaption{fig-jct-fbhd}{JCT of FBHD.}
{
}
\end{center}
\end{minipage}
\begin{minipage}{0.05in}
\hspace{0.05in}
\end{minipage}
\begin{minipage}{0.25\textwidth}
\begin{center}
\centerline{\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_Net_Queue_KV_40G.pdf}}
\vspace{-0.1in}
\mycaption{fig-queue-fbkv}{Queue Length with FBKV.}
{
}
\end{center}
\end{minipage}
\begin{minipage}{0.25\textwidth}
\begin{center}
\centerline{\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_Net_Queue_Hadoop_40G.pdf}}
\vspace{-0.1in}
\mycaption{fig-queue-hadoop}{Queue Length of FBHD.}
{
}
\end{center}
\end{minipage}
\end{figure*}
}

==> fig-NET-Real-DMAX.tex <==
{
\begin{figure}[th]
\begin{minipage}{0.5\textwidth}
\begin{minipage}{0.96\columnwidth}
\begin{center}
\centerline{\includegraphics[width=0.8\columnwidth]{new_figs/g_plot_Net_DMAX}}
\end{center}
\end{minipage}
\vspace{-0,1in}
\mycaption{fig-dmax}{fig-dmax.}
{ 
%\url{https://docs.google.com/spreadsheets/d/1Hmmr_eGg7irHsv39a5Or2sAFTTF5O-gIx7THEkiFC5s/edit#gid=1867234295}
}
\end{minipage}
\end{figure}
}


==> fig-NET-Real-EMAX-DMAX.tex <==
{
\begin{figure*}[th]
\begin{minipage}{0.33\textwidth}
\begin{minipage}{0.96\columnwidth}
\begin{center}
\centerline{\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_Net_EMAX_Batch}}
\end{center}
\end{minipage}
\vspace{-0.1in}
\mycaption{fig-emax-batch}{Accuracy and JCT with Error Budget on Spark.}
{ 
%\url{https://docs.google.com/spreadsheets/d/1Hmmr_eGg7irHsv39a5Or2sAFTTF5O-gIx7THEkiFC5s/edit\#gid=1909587585}
}
\end{minipage}
%\vspace{0.01in}
\begin{minipage}{0.33\textwidth}
\begin{minipage}{0.96\columnwidth}
\begin{center}
\centerline{\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_Net_EMAX_Stream}}
\end{center}
\end{minipage}
\vspace{-0.1in}
\mycaption{fig-emax-stream}{Accuracy and Banadwith Consumption with Error Budget on Flink.}
{ 
%\url{https://docs.google.com/spreadsheets/d/1Hmmr_eGg7irHsv39a5Or2sAFTTF5O-gIx7THEkiFC5s/edit\#gid=1909587585}
}
\end{minipage}
\if 0
\begin{minipage}{0.33\textwidth}
\begin{minipage}{0.96\columnwidth}
\begin{center}
\centerline{\includegraphics[width=0.8\columnwidth]{new_figs/g_plot_Net_DMAX}}
\end{center}
\end{minipage}
\vspace{-0.1in}
\mycaption{fig-dmax}{Accuracy with Time Budget.}
{ 
%\url{https://docs.google.com/spreadsheets/d/1Hmmr_eGg7irHsv39a5Or2sAFTTF5O-gIx7THEkiFC5s/edit#gid=1867234295}
}
\end{minipage}
\fi
\end{figure*}
}


==> fig-NET-Real-EMAX.tex <==
{
\begin{figure*}[th]
\begin{minipage}{0.24\textwidth}
\begin{minipage}{1.0\columnwidth}
\begin{center}
\centerline{\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_Net_EMAX_Batch}}
\end{center}
\end{minipage}
\vspace{-0,1in}
\mycaption{fig-emax-batch}{\sysname\ batch mode with $e_{max}$.}
{ 
%\url{https://docs.google.com/spreadsheets/d/1Hmmr_eGg7irHsv39a5Or2sAFTTF5O-gIx7THEkiFC5s/edit\#gid=1909587585}
}
\end{minipage}
%\vspace{0.01in}
\begin{minipage}{0.24\textwidth}
\begin{minipage}{1.0\columnwidth}
\begin{center}
\centerline{\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_Net_EMAX_Stream}}
\end{center}
\end{minipage}
\vspace{-0,1in}
\mycaption{fig-emax-stream}{\sysname\ streaming mode with $e_{max}$.}
{ 
%\url{https://docs.google.com/spreadsheets/d/1Hmmr_eGg7irHsv39a5Or2sAFTTF5O-gIx7THEkiFC5s/edit\#gid=1909587585}
}
\end{minipage}
\end{figure*}
}


==> fig-NET-Real-bandwidth.tex <==
{
\begin{figure}[th]
\begin{minipage}{0.5\textwidth}
\begin{minipage}{0.96\columnwidth}
\begin{center}
\centerline{\includegraphics[width=0.8\columnwidth]{new_figs/g_plot_Net_STREAM_BANDWIDTH}}
\end{center}
\end{minipage}
\vspace{-0,1in}
\mycaption{fig-stream-bw}{fig-stream-bw.}
{ 
%\url{https://docs.google.com/spreadsheets/d/1Hmmr_eGg7irHsv39a5Or2sAFTTF5O-gIx7THEkiFC5s/edit#gid=1123965524}
}
\end{minipage}
\end{figure}
}


==> fig-accurate-goodput.tex <==
{
\begin{figure}[th]
\begin{minipage}{1.0\columnwidth}
\begin{minipage}{0.48\columnwidth}
\begin{center}
\centerline{\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_ATP_accurateflow-goodput-fb.pdf}}
\vspace{-0.1in}
\mycaption{fig-rtx-fb}{Facebook}
{
The goodput of accurate flows running with approximate flows over fattree topology with Facebook workload.
\msr=0.875.
}
\end{center}
\end{minipage}
\hspace{0.01in}
\begin{minipage}{0.48\columnwidth}
\begin{center}
\centerline{\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_ATP_accurateflow-goodput-dm.pdf}}
\vspace{-0.1in}
\mycaption{fig-rtx-dm}{DM}
{
The goodput of accurate flows running with approximate flowsover fattree topology with DM workload.
\msr=0.875.
}
\end{center}
\end{minipage}
\end{minipage}
\end{figure}
}


==> fig-accurate-rtx.tex <==
{
\begin{figure}[th]
\begin{minipage}{1.0\columnwidth}
\begin{minipage}{0.48\columnwidth}
\begin{center}
\centerline{\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_ATP_accurateflow-rtx-fb.pdf}}
\vspace{-0.1in}
\mycaption{fig-rtx-fb}{Facebook}
{
The average loss rate of accurate flows running with approximate flows over fattree topology with Facebook workload.
\msr=0.875.
}
\end{center}
\end{minipage}
\hspace{0.01in}
\begin{minipage}{0.48\columnwidth}
\begin{center}
\centerline{\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_ATP_accurateflow-rtx-dm.pdf}}
\vspace{-0.1in}
\mycaption{fig-rtx-dm}{DM}
{
The average loss rate of accurate flows running with approximate flowsover fattree topology with DM workload.
\msr=0.875.
}
\end{center}
\end{minipage}
\end{minipage}
\end{figure}
}


==> fig-atpudp-lossrate-coexisting-accurate-flow.tex <==
{
\begin{figure*}[th]
\begin{minipage}{0.5\textwidth}
\begin{minipage}{0.48\textwidth}
\begin{center}
\centerline{\subfloat[\bf Approximate flows]{\label{fig-approx-queue-jct}\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_ATP_approx-jct-queue.pdf}}}
\vspace{-0.01in}
\end{center}
\end{minipage}
\begin{minipage}{0.48\columnwidth}
\begin{center}
\centerline{\subfloat[\bf Accurate flows]{\label{fig-accurate-queue-jct}\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_ATP_accurate-jct-queue.pdf}}}
\vspace{-0.1in}
\end{center}
\end{minipage}
\mycaption{fig-switch-queue-length-fattree}
{Performance Impact on Switch Drop Threshold}
{
%We study the impact of switch drop threshold of \atp\ 
%on its \jct\ and the coexisting
%accurate traffic's \jct\ using facebook workload.
}
\end{minipage}
\begin{minipage}{0.05in}
\hspace{0.05in}
\end{minipage}
\begin{minipage}{0.5\textwidth}
\begin{minipage}{0.48\columnwidth}
\begin{center}
\centerline{\subfloat[\bf Facebook]{\label{fig-accurate-fb}\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_ATP_accurateflow-loss-5.pdf}}}
\vspace{-0.1in}
\end{center}
\end{minipage}
%\vspace{-0.1in}
\begin{minipage}{0.48\columnwidth}
\begin{center}
\centerline{\subfloat[\bf DM]{\label{fig-accurate-dm}\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_ATP_accurateflow-loss-15.pdf}}}
\vspace{-0.1in}
\end{center}
\end{minipage}
\mycaption{fig-accurateflow}{Performance Impact on Accurate Flows}
{	
%Y axis shows the \jct\ of accurate flows when running with \atp\, 
%\uniformsend\, and \earlysend, and 
\msr\ is 0.875 for all tests. 
Switch buffer size is 100 and 1000 MTUs (-100 and -1000).
}
\end{minipage}
\end{figure*}
}




==> fig-batch-small-exp-delay-error-result.tex <==
{
\begin{figure}[th]
\begin{minipage}{0.5\textwidth}
\begin{minipage}{0.96\columnwidth}
\begin{center}
\centerline{\includegraphics[width=1.0\columnwidth]{new_figs/atp_small_exp_batch_delay_msr_error}}
\end{center}
\end{minipage}
\mycaption{fig-atp-small-exp-batch-delay-error}{\bf \sysname\ with user-specified \msr; Actual \jct\ and acutal error}
{ 
We ran an approximated batch aggregation job with a 15000 records dataset 
from New York taxi itinerary trace 
over a small-scale cluster. 
Users can specify both target $d_{max}$ and $e_{max}$, 
and expect the job can be finished within $d_{max}$ and 
its actual error is not over $e_{max}$
}
\end{minipage}
\end{figure}
}


==> fig-batch-small-exp-gp-jct-error-result.tex <==
{
\begin{figure*}[th]
\begin{minipage}{1.0\textwidth}
\begin{minipage}{0.33\columnwidth}
\begin{center}
\centerline{\subfloat[\bf \sysname\ with user-specified \msr]{
\label{fig-atp-small-exp-batch-gp-msr-error}
\includegraphics[width=1.0\columnwidth]{new_figs/atp_small_exp_batch_gp_msr_error.pdf}}}
%\vspace{-0.1in}
\end{center}
\end{minipage}
\hspace{0.05in}
\begin{minipage}{0.33\columnwidth}
\begin{center}
\centerline{\subfloat[\bf \uniformsend\ with user-specified \msr]{
\label{fig-ud-small-exp-batch-gp-msr-error}
\includegraphics[width=1.0\columnwidth]{new_figs/ud_small_exp_batch_gp_msr_error.pdf}}}
%\vspace{-0.1in}
\end{center}
\end{minipage}
\hspace{0.05in}
\begin{minipage}{0.33\columnwidth}
\begin{center}
\centerline{\subfloat[\bf \sysname\ with user-specified $e_{max}$]{
\label{fig-atp-small-exp-batch-gp-err-error}
\includegraphics[width=1.0\columnwidth]{new_figs/atp_small_exp_batch_gp_err_error.pdf}}}
%\vspace{-0.1in}
\end{center}
\end{minipage}
\mycaption{fig-small-exp-batch-gp-jct}{
\jct\ and acutal error}
{ 
We ran an approximated batch aggregation job with a 100000 records input dataset from  
New York taxi itinerary trace over a small-scale cluster.
We use stratefied sampling
Users can specify a target \msr\ or $e_{max}$ and expect to achieve the minimum \jct.
}
\end{minipage}
\end{figure*}
}


==> fig-batch-small-exp-msr-error-result.tex <==
{
\begin{figure*}[th]
\begin{minipage}{1.0\textwidth}
\begin{minipage}{0.33\columnwidth}
\begin{center}
\centerline{\subfloat[\bf \sysname\ with user-specified \msr]{
\label{fig-atp-small-exp-batch-msr-error}
\includegraphics[width=1.0\columnwidth]{new_figs/atp_small_exp_batch_msr_error.pdf}}}
%\vspace{-0.1in}
\end{center}
\end{minipage}
\hspace{0.05in}
\begin{minipage}{0.33\columnwidth}
\begin{center}
\centerline{\subfloat[\bf \uniformsend\ with user-specified \msr]{
\label{fig-ud-small-exp-batch-msr-error}
\includegraphics[width=1.0\columnwidth]{new_figs/ud_small_exp_batch_msr_error.pdf}}}
%\vspace{-0.1in}
\end{center}
\end{minipage}
\hspace{0.05in}
\begin{minipage}{0.33\columnwidth}
\begin{center}
\centerline{\subfloat[\bf \sysname\ with user-specified $e_{max}$]{
\label{fig-atp-small-exp-batch-err-error}
\includegraphics[width=1.0\columnwidth]{new_figs/atp_small_exp_batch_err_error.pdf}}}
%\vspace{-0.1in}
\end{center}
\end{minipage}
\mycaption{fig-small-exp-batch-msr-err-jct}{
\jct\ and acutal errors}
{ 
We ran an approximated batch aggregation job with a 100000 records input dataset 
from New York taxi itinerary trace over a small-scale cluster.
Users can specify \msr\ or $e_{max}$ and expect to achieve the minimum \jct.
}
\end{minipage}
\end{figure*}
}


==> fig-micro-params-conf.tex <==
{
\begin{figure}[th]
\begin{minipage}{1.0\columnwidth}
\begin{minipage}{0.47\columnwidth}
\begin{center}
\centerline{\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_ATP_R_min_fair_jct.pdf}}
\vspace{-0.1in}
\mycaption{fig-param-R-min}{\bf Minimum Sending Rate $R_{max}$}
{
The impact of $M$ on \atp\ fairness using microbenchmarks where \msr=0.875.
}
\end{center}
\end{minipage}
\hspace{0.1in}
\begin{minipage}{0.47\columnwidth}
\begin{center}
\centerline{\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_ATP_drop_thresh_jct.pdf}}
\vspace{-0.1in}
\mycaption{fig-param-drop-thresh}{\bf Switch Drop Threshold $q_d$}
{
The impact of $q_d$ on \jct\ using microbenchmarks where \msr=0.875.
}
\end{center}
\end{minipage}
\end{minipage}
\end{figure}
}


==> fig-network-design.tex <==
{
\begin{figure}[th]
\begin{center}
\centerline{\includegraphics[width=1.0\columnwidth]{Figures/TransportDesignChoices.pdf}}
\vspace{-0.05in}
\mycaption{f:inNetworkDesign}{Implications of Transport and Network Configuration Choices.}
{
\theo{do we want to remove Reliable/Un-Reliable from the figure? should we add a few rectangles for approximate traffic in (C)?}
}
\end{center}
\end{figure}
}


==> fig-optimization.tex <==
{
\begin{figure}[th]
\begin{minipage}{0.5\textwidth}
\begin{minipage}{0.48\columnwidth}
\begin{center}
\centerline{\subfloat[\bf Packet Loss Rate]{\label{fig-pkt-loss}\includegraphics[width=0.9\columnwidth]{new_figs/g_plot_ATP_ATPUDP-allinone.pdf}}}
\vspace{-0.01in}
\end{center}
\end{minipage}
\begin{minipage}{0.48\columnwidth}
\begin{center}
\centerline{\subfloat[\bf \jct]{\label{fig-jct}\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_ATP_ATPUDP-JCT.pdf}}}
\vspace{-0.1in}
\end{center}
\end{minipage}
\mycaption{fig-atpudp-loss-jct}
{Measured Packet Loss Rate and \jct\ of \atp\ and UDP}
{
%X axis shows the application-specified max loss rate and 
%Y axis plots the actual loss rate measured at receivers.
We meausred the packet loss rates and \jct\ of \atp\ and 
UDP with differnet \msr\ over a 192 hosts Fat-Tree topology. 
%For comparison, we also measured the average loss rate when sending UDP traffic.
}
\end{minipage}

\if 0
\begin{minipage}{0.5\textwidth}
\begin{minipage}{0.48\columnwidth}
\begin{center}
\centerline{\subfloat[\bf Facebook]{\label{fig-atp-uniformity-facebook}\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_ATP_uniformity_facebook.pdf}}}
\vspace{-0.1in}
\end{center}
\end{minipage}
%\vspace{-0.1in}
\begin{minipage}{0.48\columnwidth}
\begin{center}
\centerline{\subfloat[\bf DM]{\label{fig-atp-uniformity-dm}\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_ATP_uniformity_DM.pdf}}}
\vspace{-0.1in}
\end{center}
\end{minipage}
\mycaption{fig-Uniformity}
{Impact of Uniformity on Application Performance}
{
Each line shows a different \msr\ value.
}
\end{minipage}
\fi
\end{figure}
}



==> fig-stream-small-exp-gp-jct-error-result.tex <==
{
\begin{figure*}[th]
\begin{minipage}{1.0\textwidth}
\begin{minipage}{0.33\columnwidth}
\begin{center}
\centerline{\subfloat[\bf \sysname\ with user-specified \msr]{
\label{fig-atp-small-exp-stream-gp-msr-error}
\includegraphics[width=1.0\columnwidth]{new_figs/atp_small_exp_stream_gp_msr_error.pdf}}}
%\vspace{-0.1in}
\end{center}
\end{minipage}
\hspace{0.05in}
\begin{minipage}{0.33\columnwidth}
\begin{center}
\centerline{\subfloat[\bf \uniformsend\ with user-specified \msr]{
\label{fig-ud-small-exp-stream-gp-msr-error}
\includegraphics[width=1.0\columnwidth]{new_figs/ud_small_exp_stream_gp_msr_error.pdf}}}
%\vspace{-0.1in}
\end{center}
\end{minipage}
\hspace{0.05in}
\begin{minipage}{0.33\columnwidth}
\begin{center}
\centerline{\subfloat[\bf \sysname\ with user-specified $e_{max}$]{
\label{fig-atp-small-exp-stream-gp-err-error}
\includegraphics[width=1.0\columnwidth]{new_figs/atp_small_exp_stream_gp_err_error.pdf}}}
%\vspace{-0.1in}
\end{center}
\end{minipage}
\mycaption{fig-small-exp-stream-gp-jct}{
Bandwidth consumption and acutal error}
{ 
We ran an approximated streaming aggregation job 
with a 5s tumbling time window over a small-scale cluster. 
We use stratified sampling.
Producers generate and send records from the New York taxi itinerary trace.
Users can specify a target \msr\ or $e_{max}$
}
\end{minipage}
\end{figure*}
}


==> fig-stream-small-exp-jct-error-result.tex <==
{
\begin{figure*}[th]
\begin{minipage}{1.0\textwidth}
\begin{minipage}{0.33\columnwidth}
\begin{center}
\centerline{\subfloat[\bf \sysname\ with user-specified \msr]{
\label{fig-atp-small-exp-stream-msr-error}
\includegraphics[width=1.0\columnwidth]{new_figs/atp_small_exp_stream_msr_error.pdf}}}
%\vspace{-0.1in}
\end{center}
\end{minipage}
\hspace{0.05in}
\begin{minipage}{0.33\columnwidth}
\begin{center}
\centerline{\subfloat[\bf \uniformsend\ with user-specified \msr]{
\label{fig-ud-small-exp-stream-msr-error}
\includegraphics[width=1.0\columnwidth]{new_figs/ud_small_exp_stream_msr_error.pdf}}}
%\vspace{-0.1in}
\end{center}
\end{minipage}
\hspace{0.05in}
\begin{minipage}{0.33\columnwidth}
\begin{center}
\centerline{\subfloat[\bf \sysname\ with user-specified $e_{max}$]{
\label{fig-atp-small-exp-stream-err-error}
\includegraphics[width=1.0\columnwidth]{new_figs/atp_small_exp_stream_err_error.pdf}}}
%\vspace{-0.1in}
\end{center}
\end{minipage}
\mycaption{fig-small-exp-stream-jct}{
Bandwidth consumption and acutal error}
{ 
We ran an approximated streaming aggregation job with a 5s tumbling time window 
over a small-scale cluster. 
Producers generate and send records from the New York taxi itineray trace.
Users can specify a target \msr\ or $e_{max}$
}
\end{minipage}
\end{figure*}
}


==> fig-toy-example-atp-fct-queue.tex <==
{
\begin{figure}[th]
\begin{minipage}{0.5\textwidth}
\begin{minipage}{0.48\columnwidth}
\begin{center}
\centerline{\subfloat[\bf 1Gbps]{
\label{fig-toy-fct-queue-1g}
\includegraphics[width=1.0\columnwidth]{new_figs/atp_toy_num_flow_fct_queue.pdf}}}
\end{center}
\end{minipage}
\begin{minipage}{0.48\columnwidth}
\begin{center}
\centerline{\subfloat[\bf 10Gbps]{
\label{fig-toy-fct-queue-10g}
\includegraphics[width=1.0\columnwidth]{new_figs/atp_toy_num_flow_fct_queue_10g.pdf}}}
\end{center}
\end{minipage}
\mycaption{fig-toy-fct-queue}{\fct\ and Queueing Length}
{ 
We ran a microbenchmark comparing the \fct\ and queueing length of \atp\
to \dctcp\ \earlysend\ over a controlled network with a (a) 1Gbps and 
(b) 10Gbps bottleneck link respectively.
}
\end{minipage}
\end{figure}
}


==> fig-waterfall.tex <==
{
\begin{figure}[th]
\begin{center}
\centerline{\includegraphics[width=1.0\columnwidth]{Figures/WaterFallDesignChoices.pdf}}
\vspace{-0.05in}
\mycaption{f:aproxcomp:waterfall}{Comparison of Different Approximate Computing Schemes.}
{
Waterfall of stages in data transfer.
}
\end{center}
\end{figure}
}


==> fig-workflow.tex <==
{
\begin{figure}
\begin{center}
\centerline{\includegraphics[width=0.95\columnwidth]{new_figs/foglight_workflow.pdf}}
\vspace{-0.05in}
\mycaption{fig-flow}{\sysname\ Workflow.}
{
\sysname\ has three stages: 1) define jobs and approximation semantics, 
2) transmit messages using \atp, and 3) estimate result accuracy with confidence interval.
}
\end{center}
\end{figure}
%\vspace{-0.1in}
}


==> fig-workload-completion-time-with-job-arrival-rate.tex <==
{
\begin{figure*}[th]
\begin{minipage}{1.0\textwidth}
\begin{minipage}{0.24\columnwidth}
\begin{center}
\centerline{\subfloat[\bf Facebook 1\gbps]{\label{fig-workload-fb-tl-1g}\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_ATP_workload-Facebook-TL.pdf}}}
\vspace{-0.1in}
\end{center}
\end{minipage}
%\vspace{-0.1in}
\begin{minipage}{0.24\columnwidth}
\begin{center}
\centerline{\subfloat[\bf Facebook 10\gbps]{\label{fig-workload-fb-tl-10g}\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_ATP_workload-Facebook-10G-TL.pdf}}}
\vspace{-0.1in}
\end{center}
\end{minipage}
\begin{minipage}{0.24\columnwidth}
\begin{center}
\centerline{\subfloat[\bf DM 1\gbps]{\label{fig-workload-mining-tl-1g}\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_ATP_workload-Mining-TL.pdf}}}
\vspace{-0.1in}
\end{center}
\end{minipage}
\begin{minipage}{0.24\columnwidth}
\begin{center}
\centerline{\subfloat[\bf DM 10\gbps]{\label{fig-workload-mining-tl-10g}\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_ATP_workload-Mining-10G-TL.pdf}}}
\vspace{-0.1in}
\end{center}
\end{minipage}
\mycaption{fig-workload-completion-time-job-arrival-rate}
{JCT with Different Traffic Load}
{
Facebook and data mining workloads running on 
1\gbps\ ((a) and (c)) and 
10\gbps\ ((b) and (d)) network.
%Traffic load means  
}
\end{minipage}
\end{figure*}
}


==> fig-workload-completion-time-with-max-loss-rate.tex <==
{
\begin{figure*}[th]
\begin{minipage}{1.0\textwidth}
\begin{minipage}{0.24\columnwidth}
\begin{center}
\centerline{\subfloat[\bf Facebook 1\gbps]{\label{fig-workload-fb-ml-1g}\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_ATP_workload-Facebook-ML.pdf}}}
\vspace{-0.1in}
\end{center}
\end{minipage}
%\vspace{-0.1in}
\begin{minipage}{0.24\columnwidth}
\begin{center}
\centerline{\subfloat[\bf Facebook 10\gbps]{\label{fig-workload-fb-ml-10g}\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_ATP_workload-Facebook-10G-ML.pdf}}}
\vspace{-0.1in}
\end{center}
\end{minipage}
\begin{minipage}{0.24\columnwidth}
\begin{center}
\centerline{\subfloat[\bf DM 1\gbps]{\label{fig-workload-mining-ml-1g}\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_ATP_workload-Mining-ML.pdf}}}
\vspace{-0.1in}
\end{center}
\end{minipage}
\begin{minipage}{0.24\columnwidth}
\begin{center}
\centerline{\subfloat[\bf DM 10\gbps]{\label{fig-workload-mining-ml-10g}\includegraphics[width=1.0\columnwidth]{new_figs/g_plot_ATP_workload-Mining-10G-ML.pdf}}}
\vspace{-0.1in}
\end{center}
\end{minipage}
\mycaption{fig-workload-completion-time-max-loss-rate}{JCT with Different \msr}
{ 
We ran Facebook and data mining (DM) workload over a 192 hosts Fat-Tree
topology with 1\gbps\ ((a) and (c)) and 10\gbps\ ((b) and (d)) 
link capacity. 
}
\end{minipage}
\end{figure*}
}


==> introduction.tex <==
\section{Introduction}
\label{sec:introduction}
Many popular data analytics and machine learning applications, \eg, workloads running on Spark, TensorFlow, and Kafka, 
which dominate data centers, are capable of delivering highly accurate results by processing only a subset of their input data.
This principle is commonly known as \textit{Approximate Computing}~\cite{Baek10-PLDI, Bornholt-ASPLOS14,Sampson11-PLDI, Sampson13-MICRO,Agarwal13-EUROSYS, Ananthanarayanan14-NSDI, Chaudhuri07-IEEE, 
Condie10-NSDI, Goiri-Asplos15, Hellerstein97-SIGMOD, Pansare11-PVLDB, 
StreamApprox2017,Chris-VLDB08}: 
computation is performed over incomplete data to provide an approximate answer 
but with faster response times and/or lower resource footprint. 
Motivated by the observation that approximate computing workloads contain inherent slack, 
both in the data and in the processing of said data, there has been extensive work at 
the programming language~\cite{Baek10-PLDI, Bornholt-ASPLOS14,Sampson11-PLDI, Sampson13-MICRO}, 
hardware ~\cite{Sampson13-MICRO}, storage ~\cite{Sampson13-MICRO}, 
and application ~\cite{Agarwal13-EUROSYS, Ananthanarayanan14-NSDI, Chaudhuri07-IEEE, 
Condie10-NSDI, Goiri-Asplos15, Hellerstein97-SIGMOD, Pansare11-PVLDB, 
StreamApprox2017,Chris-VLDB08} levels to better utilize this slack to minimize resource utilization, 
improve performance and reduce the energy used by these workloads.

Most datacenter approximate applications run on a distributed set of machines and involve network communication. 
Unfortunately and surprisingly, there has been almost no work that considers approximate computing together with the network layer.
Distributed approximate applications treat the network as a black box,
and the network is, in turn, oblivious of approximate traffic and its inherent tolerance to slack.
As a result, today's approximate applications leverage their slack at the application level either by sampling (i.e., dropping) data at the sender before sending over a reliable network~\cite{Goiri-Asplos15}, or by sampling at the receiver side~\cite{StreamApprox2017} (i.e., dropping a subset of received data at the transport layer before delivery to the application).
Meanwhile, the reliable network aims to deliver each and every packet even when there is loss. %could experience packet loss and has to retransmit the lost data.
Instead of treating the network as a black box, would it be beneficial to make \textit{approximate computing network-aware} and the \textit{network 
approximate-computing aware}?
%Our key insight is that 
%Intuitively, approximate applications could tolerate loss
%the network could drop packets
%treats approximate and non-approximate traffic in the same way.
% at the network layer, there has been little work to leverage the unique properties of 
%approximate computing to improve network utilization and effectiveness. 
%Additionally, approximate applications are network unaware,
%missing the opportunities to leverage network state to improve application performance.
%We argue and show that there is a significant benefit to \textit{making network 
%approximate-computing aware} and \textit{making approximate computing network-aware}. 
%Our work aims to fill this gap by using the slack inherent in approximate applications 
%to rethink network resource allocation and application communication design. 
%In particular, our work is motivated by the following two questions: 

More specifically, we ask ``\textit{Is it possible for approximate applications to leverage 
network state to improve performance without loss of accuracy?}'',
and ``\textit{Is it possible for the network to leverage the inherent slack 
in approximate application to improve network resource allocation?}''?


Our answer to these questions is {\em \sysname}, 
a new approximate-computing-aware network system that includes %a transport-layer protocol, 
%resource allocation algorithms at the switch queuing layer.
%new scheduling algorithms, and new switch queuing 
%an ensemble of 
protocol, scheduling, and resource allocation algorithms 
at the transport and switch queuing layers.
\sysname\ not only improves the performance of approximate applications (with guaranteed application accuracy)
but also frees up network resources for non-approximate traffic, which in turn improves the performance of non-approximate applications. 
\sysname's core insights that due to approximate applications' inherent ability to tolerate loss, we can (1) send approximate traffic aggressively but in a network-aware and approximate-application-aware way,
and (2) allocate tiny switch buffers for approximate traffic.  

Although these high-level ideas are simple, there are several critical challenges in realizing them \theo{in a general manner that supports the broad range of approximate applications from streaming and batch to deep learning}.
First, although approximate applications can tolerate some slack, dropping data arbitrarily is not acceptable as these applications still have certain accuracy requirements. 
\sysname\ needs to accurately infer the approximation slack \theo{in an application-agnostic manner} and deliver optimal performance without violating accuracy requirements.
%, which is both application and workload-specific, 
Second, \sysname\ needs to automatically and effectively react to dynamic network 
variability by adjusting the approximate traffic's behavior (i.e., sampling and sending rate).
Third, \sysname\ should smartly allocate network resources to non-approximate traffic and approximate traffic with different accuracy requirements,
in a way that is ``fair'', efficient, and free of starvation.  \theo{Addressing these challenges with an application-specific point-solution is trivial, however, providing a general application requires exploring designs that span across multiple layers of the network.}

To solve these challenges, we propose a set of \emph{slack-based} network techniques,
including a slack-based adaptive congestion control algorithm, a slack-based switch resource allocation mechanism, a slack-based switch queue assignment policy, .


The core of \sysname\ is the {\em Approximate Transmission Protocol}, or {\em \atp}, a new transport-layer protocol 
designed for datacenter approximate applications. % (Section~\ref{sec:design}).
\atp\ opportunistically utilizes all available network bandwidth assigned to approximate traffic 
by aggressively sending data as early and as fast as allowed by application requirements and network congestion state.
\theo{The core of \sysname\ is the {\em Approximate Transmission Protocol}, or {\em \atp}, a principled approach for redesigning existing transport-layer protocol for datacenter approximate applications. % (Section~\ref{sec:design}).
\atp\ incorporates slack into an existing transport and enables it to opportunistically utilize all available network bandwidth assigned to approximate traffic 
by aggressively sending data as early and as fast as allowed by application requirements and network congestion state. }
We design a {\em loss-based} congestion control mechanism which uses \emph{loss as the congestion measurement},
dynamically adjusting a \emph{target loss rate} based on the congestion measurement,
and quickly adapts the sending rate to accommodate this target loss rate.
\theo{We demonstrate the feasibility of \atp by enhancing a {\em loss-based} congestion control mechanism which uses \emph{loss as the congestion measurement}, to 
dynamically incorporate a \emph{target loss rate} based on the congestion measurement,
and quickly adapt the sending rate to accommodate this target loss rate.}
We further employ a scheduling algorithm which leverages approximate applications' relaxed ordering requirement 
to possibly send messages out of order for better performance. 
Together, these techniques ensure minimal retransmission, efficient bandwidth utilization, and fast job completion.

Another core design of \sysname\ is its \emph{loss-based network resource allocation} at the switch level.
\sysname\ leverages separate switch priority queues to categorize non-approximate traffic and approximate traffic with different accuracy requirements.
\sysname\ configures lower-priority queues to a tiny queue size and associate approximate flows with more loss tolerance to these queues.
The highest priority queue and almost all switch buffer space are reserved for non-approximate traffic.
These switch settings improves the performance of non-approximate workloads while not affecting the performance or accuracy of approximate workloads.
%For approximate traffic, \sysname\ uses a near-zero switch queue which works well together with \atp\ 
%and almost all switch buffer space for non-approximate traffic.
%\sysname\ only requires switch configuration changes and works with all existing load-balancing and routing schemes.

On top of \atp, \sysname\ includes a developer-friendly user-level library, {\em \approxlib}, which acts as a bridge between the stream/batch frameworks and our approximate transport (\atp).
\approxlib\ makes it easy for applications to allocate minimal \sysname\ and specify their sampling strategies.

We evaluated \sysname\ by using a combination of large-scale simulations to understand our techniques under production scales 
and a testbed with four popular batch and streaming frameworks to understand practical deployment challenges. 
In our simulation, we evaluated \sysname\ using large Fat-Tree~\cite{Al-Fares-Sigcomm08} and Leaf-Spine topologies
and two real-world traces, a Facebook key-value store workload~\cite{Atikoglu12-keyvalueanal}
and a Facebook Hadoop workload~\cite{Roy-Sigcomm15}. \theo{Is a leaf-spine topology a different term for a two-tier clos topology? e.g., Microsoft's Vl2?}
We compared \sysname\ to UDP, DCTCP~\cite{Alizadeh10-SIGCOMM}, pFabric~\cite{Alizadeh-Sigcomm13}, and two sender-drop approaches, 
one that drops packets uniformly throughout a job and one that sends data as early as possible.
We ported four data-processing frameworks, Kafka~\cite{apach-kafka}, Flink~\cite{apach-flink}, Spark~\cite{apach-spark}, and PyTorch~\cite{PyTorch}
to our real implementation of \sysname.
We evaluated these systems with four real-world workloads and three types of approximate computing algorithms.
Our evaluation results show that 
\sysname\ improves application job completion time by up to 80\%.
Meanwhile, \sysname's measured loss rate is small %(at most 9\%) 
and always below application-specified max loss rate.
Moreover, it achieves fairness across different (approximate and non-approximate) jobs and improves the performance of co-running non-approximate traffic by 79\%.

This paper makes the following contribution.

\vspace{-0.05in}
\begin{itemize}
\vspace{-0.05in}
\item Analysis of the limitations of existing approximation systems that are network oblivious.
\vspace{-0.05in}
\item The first proposal of incorporating approximate computing at the network layer. % and we identified the advantages and challenges of doing so.
\vspace{-0.05in}
\item \atp, a new transport protocol designed for distributed approximate computing, and a set of approximate-aware switch resource allocation policies. 
\vspace{-0.05in}
\item A approximate library that works for common types of data-processing and machine-learning applications.
\vspace{-0.05in}
\item Implementation of \sysname\ with both simulation and real implementation, and four real datacenter distributed frameworks ported to \sysname.
\vspace{-0.05in}
\end{itemize}
\vspace{-0.05in}

We will make our simulation and real implementation source code publicly available soon.





==> related.tex <==
\section{Related Work}
\label{sec:related}

This section discusses work that is related to \sysname.
%\sysname\ builds on two paradigms, namely,
%approximate computing and datacenter networking 
%including congestion control, flow scheduling and 
%load balancing.
%In this section, we survey the techniques proposed in these two paradigms.

\boldparagraph{Approximate computing systems.}
%Given the advantages of making a tradeoff between accuracy and efficiency, 
As more types of applications such as machine learning and data analytics can tolerate approximation,
extensive efforts have been investigated in applying approximate techniques at different systems levels, 
from programming language \cite{Sampson11-PLDI, Baek10-PLDI} and hardware~\cite{Sampson13-MICRO}
to query and database systems~\cite{Agarwal13-EUROSYS, Chaudhuri07-IEEE,Chris-VLDB08}. 
There are also approximate systems designed for different types of 
%They also applied approximation on 
data-processing systems such as Hadoop, MapReduce, and 
data streaming systems\cite{Condie10-NSDI, Pansare11-PVLDB, 
Hellerstein97-SIGMOD, Ananthanarayanan14-NSDI, Goiri-Asplos15, StreamApprox2017}.
They focus on reducing the application running time by applying 
approximations on application algorithms. 
All of them run on a reliable network and perform approximate tasks
at host machines (usually at receiving nodes that perform the actual computation).
There are some proposals~\cite{SAP15, Fujuki17-IEEE, Sen-Sigcomm10}
to relax network integrity checks (\ie, allowing bit errors) for approximate applications.
They focus on low-level network properties and target wireless and optical network.
\sysname\ is the first proposal to apply integrate approximation and datacenter network transport layer.
It not only improves the performance of approximate applications
but also leaves more network resources for co-running non-approximate applications.
% approximations in network transmissions 
%to reduces the communication delay in terms of JCT.

\if 0
There have been a host of systems that leverage the approximation nature
in many types of applications to improve performance~\cite{Agarwal13-EUROSYS, Chaudhuri07-IEEE, Chris-VLDB08, 
Condie10-NSDI, Pansare11-PVLDB, Hellerstein97-SIGMOD, 
Ananthanarayanan14-NSDI, Goiri-Asplos15, StreamApprox2017,
Xin-OSDI18,IncApprox-WWW16,ApproxJoin-SoCC18,Haoyu-NSDI17, 
Park-SIGMOD18, Kandula-SIGMOD16}.
As a result, 
their approximation algorithms are confined within host machines, 
and result in bandwidth waster by blindly sending complete datasets. 
In contrast, 
\sysname\ takes the first step to apply approximations (sampling) 
during network communications to 
reduces the communication delay in terms of \jct, 
while guarantees the job accuracy by controlling the data loss rate. 
Although the goals of \sysname 's and existing approximate computing systems
might overlap, \sysname\ is largely orthogonal to those systems 
and can be used by them.
To the best of our knowledge, 
existing works~\cite{SAP15, Fujuki17-IEEE, Sen-Sigcomm10} 
applied approximation on 
network by both relaxing the lower layer integrity checking on data bit errors 
when transmitting over wireless and optical networks, 
which tradeoffs the better performance 
in terms of better resource efficiency and lower latency. 
Their approaches cannot work well over datacenter networks, 
as the bit error rate is not as significant as wireless and optical networks.   
\fi

\boldparagraph{Datacenter network design.}
%Congestion Control, Flow Scheduling 
%and Load Balancing.}
There has been a large body of work on datacenter congestion control and flow scheduling~\cite{Alizadeh-Sigcomm13, Gao-CoNext15, Alizadeh10-SIGCOMM, 
Vamanan-Sigcomm12, Wu-CoNext10, Han-Sigcomm13, Cho17-SIGCOMM, 
Mark-Sigcomm17, Behnam-Sigcomm18, Wei-nsdi15,Behnam-Sigcomm18}.
While improving flow completion time, 
they require sufficient switch buffer~\cite{Alizadeh-Sigcomm13, Gao-CoNext15, Cho17-SIGCOMM, Mark-Sigcomm17, Behnam-Sigcomm18}.
%and have presumption on the datacenter topology
%~\cite{Gao-CoNext15, Cho17-SIGCOMM, Mark-Sigcomm17, 
%Behnam-Sigcomm18}
\atp\ takes a different approach on the switch queuing problem:
leveraging the approximate computing nature to leave switch buffer space for \nonapproximate flows.
%In contrast, \sysname\ uses \atp\ which achieves zero-queueing 
%and faster convergence speed by leveraging the approximate nature.  
%\atp 's rate adaptation is inspired from the loss-rate-based rate control 
%in ExpressPass~\cite{Cho17-SIGCOMM}. 
%But ExpressPass uses it for controlling the rate of infinite, 
%small-size credit packets,
%and the received credits are used to schedule transmissions of accurate flows, 
%while \atp\ uses it in approximate computing context 
%with the goal of eliminating queueing 
%and minimizing bandwidth allocation for approximate traffic. 
Fastpass~\cite{Perry-Sigcomm14} leverages a central controller to achieve “zero-queueing”,
but the central controller limits the scalability of the system.
%with the increase scaling of datacenter workload, 
%it is difficult for a controller to schedule all datacenter traffic.

%\atp 's MRDF message scheduling is similar to flow scheduling 
%in PIAS~\cite{Wei-nsdi15}, NDP~\cite{Mark-Sigcomm17} and Homa~\cite{Behnam-Sigcomm18}, 
%all of which are inspired from shortest-remaining-processing-first, 
%but MRDF is used for approximate traffic and does not require priority queues.

%Datacenter load balancing algorithm is orthogonal to \atp.
%They are either packet-based~\cite{Alizadeh-Sigcomm13,  
%RPS, Zats-Sigcomm12, Perry-Sigcomm14}, 
%or flow/flowlet-based~\cite{Letitflow-NSDI17, Zhang-Sigcomm17, 
%FlowBender, Katta-Hotnets16, Alizadeh-Sigcomm14}. 
%Therefore, we believe \atp\ is compatible with them, 
%as we showed in Section~\ref{sec:design} that \atp\ 
%works well with ECMP~\cite{ECMP-RFC} and packet spray~\cite{RPS}.


==> remark.tex <==
\newif\ifremark
\long\def\remark#1{
\ifremark%
        \begingroup%
        \dimen0=\columnwidth
        \advance\dimen0 by -1in%
        \setbox0=\hbox{\parbox[b]{\dimen0}{\protect\em #1}}
        \dimen1=\ht0\advance\dimen1 by 2pt%
        \dimen2=\dp0\advance\dimen2 by 2pt%
        \vskip 0.25pt%
        \hbox to \columnwidth{%
                \vrule height\dimen1 width 3pt depth\dimen2%
                \hss\copy0\hss%
                \vrule height\dimen1 width 3pt depth\dimen2%
        }%
        \endgroup%
\fi}


==> tbl-sampling.tex <==
{
\begin{table}[th]\footnotesize
%\begin{minipage}{\figWidth}
\begin{center}
\begin{center}
\scriptsize
	\begin{tabular}{c|c}
		\textbf{Sampling Type} & \textbf{Specification to \approxlib} \\ \hline \hline
		
		Stratified~\cite{ApproxJoin-SoCC18, Kandula-SIGMOD16,Park-SIGMOD18, Agarwal-EUROSYS13} & same \msr\ aross different groups \\ \hline
	        Uniform~\cite{StreamApprox2017,Goiri-Asplos15} & same \msr\ for whole dataset. Uniformity is 1 \\ \hline
		Quota~\cite{Agarwal13-EUROSYS} & \msr\ is proportional to group size 
        \end{tabular}
\end{center}
\vspace{0.1in}
\mycaption{tbl-sample}{Typical Sampling Types and Their Specifications to \approxlib}
{
}
\end{center}
%\end{minipage}
%\vspace{-0.1in}
\end{table}
}



